Contextualization of ASR with LLM using phonetic retrieval-based augmentation

Large language models (LLMs) have shown superb capability of modeling multimodal signals including audio and text, allowing the model to generate spoken or textual response given a speech input. However, it remains a challenge for the model to recognize personal named entities, such as contacts in a phone book, when the input modality is speech. In this work, we start with a speech recognition task and propose a retrieval-based solution to contextualize the LLM: we first let the LLM detect named entities in speech without any context, then use this named entity as a query to retrieve phonetically similar named entities from a personal database and feed them to the LLM, and finally run context-aware LLM decoding. In a voice assistant task, our solution achieved up to 30.2% relative word error rate reduction and 73.6% relative named entity error rate reduction compared to a baseline system without contextualization. Notably, our solution by design avoids prompting the LLM with the full named entity database, making it highly efficient and applicable to large named entity databases.

==> Makefile <==
PAPER=asr_llm_contextualization
VENUE=icassp2025

all: $(VENUE)-$(PAPER).pdf

$(VENUE)-$(PAPER).pdf: *.tex *.bib
	pdflatex $(VENUE)-$(PAPER)
	bibtex $(VENUE)-$(PAPER)
	pdflatex $(VENUE)-$(PAPER)
	pdflatex $(VENUE)-$(PAPER)

clean:
	rm -Rf \
		"$(VENUE)-$(PAPER).bbl" \
		"$(VENUE)-$(PAPER).blg" \
		"$(VENUE)-$(PAPER).log" \
		"$(VENUE)-$(PAPER).aux" \
		"$(VENUE)-$(PAPER).out" \
		"$(VENUE)-$(PAPER).pdf" \
		"$(VENUE)-$(PAPER).zip"

